Mitigating Gender Bias for Neural Dialogue Generation with Adversarial Learning

Dialogue systems play an increasingly important role in various aspects of our daily life. It is evident from recent research that dialogue systems trained on human conversation data are biased. In particular, they can produce responses that reflect people's gender prejudice. Many debiasing methods have been developed for various NLP tasks, such as word embedding. However, they are not directly applicable to dialogue systems because they are likely to force dialogue models to generate similar responses for different genders. This greatly degrades the diversity of the generated responses and immensely hurts the performance of the dialogue models. In this paper, we propose a novel adversarial learning framework Debiased-Chat to train dialogue models free from gender bias while keeping their performance. Extensive experiments on two real-world conversation datasets show that our framework significantly reduces gender bias in dialogue models while maintaining the response quality. The implementation of the proposed framework is released.

==> old_introduction.tex <==
\section{Introduction}
The elimination of discrimination is an important issue that our modern-day society is facing. Learning from humans' behaviors, machine learning algorithms have been proven to inherit the prejudices from humans~\cite{mehrabi2019survey}. A variety of AI applications have demonstrated common prejudices towards particular groups of people~\cite{rodger2004field,howard2018ugly,rose2010face,yao2017beyond,DBLP:conf/icail/TolanMGC19}. It is evident from recent research that learning-based dialogue systems also suffer from discrimination problems~\cite{liu2019does,dinan2019queens}. Dialogue models show significant prejudices towards certain groups of people by producing biased responses to messages related to different genders~\cite{liu2019does}. A biased dialogue system will produce improper speeches, which can bring in bad experiences to users and can even cause negative social impacts~\cite{DBLP:journals/sigcas/WolfMG17}. Thus, with the increasing demand of using dialogue agents in our daily lives, it is highly desired for us to take the fairness issue into consideration when developing dialogue systems. 

% The elimination of discrimination is an important issue that our modern-day society is facing. Learning from humans' behaviors, machine learning algorithms have been proven to inherit the prejudices from humans~\cite{mehrabi2019survey}. From speech recognition~\cite{rodger2004field}, computer vision~\cite{howard2018ugly,rose2010face}, recommendation systems~\cite{yao2017beyond} to predictive models~\cite{DBLP:conf/icail/TolanMGC19}, a variety of AI applications have demonstrated common prejudices towards particular groups of people. It is evident from recent research that learning-based dialogue systems also suffer from discrimination problems~\cite{liu2019does,dinan2019queens}. Both neural generative models and retrieval-based models show significant prejudices towards certain groups of people by producing biased responses to messages related to different genders and races~\cite{liu2019does}. Given the increasing demand of using dialogue agents in our daily lives, it is highly desired for us to take the fairness issue into consideration when developing dialogue systems. Otherwise, a biased dialogue system will produce improper speeches, which can bring in bad experiences to users and can even cause negative social impacts~\cite{DBLP:journals/sigcas/WolfMG17}.

The gender bias in dialogues comes from different dimensions -- the gender of the person speakers are talking about (speaking-about), and the gender of the speaker (speaking-as) and the addressee (speaking-to)~\cite{DBLP:journals/corr/abs-2005-00614}. In this work, we focus on mitigating gender biases of dialogue systems in the speaking-about dimension.  It is the most common format of gender bias in dialogues which exists under both speaker-agnostic and speaker-given dialogue scenarios. Given messages with the same content for different genders, dialogue models could produce biased responses, which have been measured in terms of their politeness and sentiment, as well as the existence of biased words~\cite{liu2019does}. {\bf existing diag models are biased and use examples? }




{\bf why we need new solutions (why exisitng ones cannot be applied)?  what are the challenges for new solutions? the biggest challenge is to debias and keeping gender related features ...  }
Directly applying existing debiasing methods such as data augmentation~\cite{dinan2019queens} and word embeddings regularization~\cite{liu2019does} to mitigate the biases could  encourage dialogue models to produce the same response for different genders. This strategy can lead to producing unreasonable responses such as ``he gave birth to a baby'' and also reduce the diversity of the generated responses. For different genders, a desired dialogue model should produce responses which not only are bias-free but also comprise reasonable gender features. In other words, we should build a fair dialogue model without sacrificing its performance. 

% We could adapt existing debiasing solutions for other tasks in NLP such as coreference solution~\cite{DBLP:journals/corr/abs-1804-06876} and machine translation~\cite{DBLP:journals/corr/abs-1901-03116} to build a bias-free dialogue system. We could augment the training data by copying each dialogue in the dataset with gender words swapped~\cite{dinan2019queens}. However, this solution may cause the model to produce the same content for different genders, and perhaps only the gender words have changed. Besides, inappropriate dialogues such as ``he gave birth to a baby'' can be added to the training data and can lead to similar responses that do not make sense. We could also eliminate the differences of word embeddings of gender words during training to build a model with gender equity~\cite{liu2019does}. However, this method tends to generate bias-free but identical responses to both genders. In fact, these debiasing approaches encourage the dialogue model to produce homogeneous responses to males and females while ignoring the reasonable differences that should exist in the responses for different genders. This will reduce the diversity of the generated responses and affect the performance of the dialogue model. Therefore, dedicated efforts are desired for dialogue systems.

% Our focus in this work is to mitigate gender biases in dialogue systems. We could adapt existing debiasing solutions for other tasks in NLP such as coreference solution~\cite{DBLP:journals/corr/abs-1804-06876} and machine translation~\cite{DBLP:journals/corr/abs-1901-03116} to build a bias-free dialogue system. We could augment the training data by copying each dialogue in the dataset with gender words swapped~\cite{dinan2019queens}. However, this solution may cause the model to produce the same content for different genders, and perhaps only the gender words have changed. Besides, inappropriate dialogues such as ``he gave birth to a baby'' can be added to the training data and can lead to similar responses that do not make sense. We could also eliminate the differences of word embeddings of gender words during training to build a model with gender equity~\cite{liu2019does}. However, this method tends to generate bias-free but identical responses to both genders. In fact, these debiasing approaches encourage the dialogue model to produce homogeneous responses to males and females while ignoring the reasonable differences that should exist in the responses for different genders. This will reduce the diversity of the generated responses and affect the performance of the dialogue model. Therefore, dedicated efforts are desired for dialogue systems. {\color{blue} Shorten this paragraph.}

% \begin{figure}[!t]
% \includegraphics[width=\linewidth]{figs/intro.pdf}
% \caption{Two illustrative responses to a female-related message. The first one is unbiased while the second one could be biased.}
% \vspace{-0.3in}
% \label{fig:example}
% \end{figure}

\begin{table*}[]
\small
\centering
\caption{Examples of Gender Biases in Dialogue Systems.}
\label{tab:intro}
\begin{tabular}{|p{3cm}|p{4cm}||p{5cm}|p{3cm}|}
\hline
Message & Response & Message & Response \\ \hline
Hahaha, \textbf{he} has a really cute laugh and smile:d & He really is the sweetest. all he does is make that cute little smile. & what \textbf{he} doesnt mention is \textbf{his} specialty? so \textbf{he} is seeking for a new job?? & he ' s busy with his business . \\ \hline
Hahaha, \textbf{she} has a really cute laugh and smile:d & She cute but she is also kinda evil. & what \textbf{she} doesnt mention is \textbf{her} specialty? so \textbf{she} is seeking for a new job?? & she ' s a little bitch . \\ \hline
\end{tabular}
\end{table*}

Figure~\ref{fig:example} shows two responses to a message about a female. Though both of them contain features related to the gender, the first one is unbiased while the second one could be biased. In the first response, the word ``actress'' is a female occupation and the phrase ``natural beauty'' is only used to describe women. They are reasonable gender features and have nothing to do with gender discrimination. We refer to the reasonable and fair gender features in the responses as the \emph{unbiased gender features} of the responses. The second response contains a family-related word ``housework'', which are defined as biased words in~\cite{liu2019does}. When asking the occupation of a female, a biased response is more likely to have family-related words such as ``housework'' and ``babysit'' than the case of a male, which reflects the society's stereotype of females and belongs to the category of discrimination. We call the unreasonable and discriminatory gender features as the \emph{biased gender features} of the responses. With these two types of features, a reasonable and unbiased dialogue model should produce responses with unbiased gender features but free from biased gender features. In other words, a response of good quality should contain necessary gender-related information but should not include information reflecting sexism.

% In this paper, we aim to build a dialogue model where both fairness and performance are taken into considered. Figure~\ref{fig:example} shows two responses to a message about a female. Though both of them contain features related to the gender, the first one is unbiased while the second one could be biased. In the first response, the word ``pregnant'' is more likely to appear in a response to a message about females, which is a reasonable difference instead of discrimination because it's a natural physiological difference between males and females. We refer to the reasonable and fair differences in the responses towards different genders as the \emph{unbiased gender features} of the responses. The second response contains family words such as ``housewife'' and ``housework''. When asking the occupation of a female, a biased response is more likely to have family words such as ``housewife'' and ``housework'' than the case of a male, which reflects the society's stereotype of females and belongs to the category of discrimination. We call the unreasonable and discriminatory differences as the \emph{biased gender features} of the responses. With these two types of features, a reasonable and unbiased dialogue model should produce responses with unbiased gender features but free from biased gender features. In other words, a response of good quality should contain necessary gender-related information but should not include information reflecting sexism.

{\bf briefly state we have done and what are our contributions? }

In order to build a dialogue model that can produce responses meeting the above requirements, we face two key challenges. First, since biases have many forms and are defined subjectively, it's hard for us to delimit the unbiased and biased gender features of a given utterance. Second, if we can get the unbiased and biased gender features, it is difficult to utilize them to guide the training of a bias-free dialogue model. To solve the first challenge, we propose a disentanglement model that learns to separate the unbiased gender features from the biased gender features of a gender-related utterance. Then, for the second challenge, we propose an adversarial learning framework to train bias-free generative dialogue models which produce responses with unbiased gender features and without biased gender features. We empirically validate the effectiveness of our proposed framework {\bf Debiased-Chat} by conducting experiments on two real-world dialogue datasets. Results show that our method can significantly mitigate the gender biases in generative dialogue models while maintaining the performance of the dialogue model to produce engaging and diverse responses with distinctive unbiased gender features.

% However, we face two key challenges to achieve the latter goal. First, since biases have many forms and are defined subjectively, it's hard for us to delimit the unbiased and biased gender features of a given utterance. Second, if we can get the unbiased and biased gender features, it is difficult to utilize them to guide the training of a bias-free dialogue model.  To solve the first challenge, we propose a disentanglement model that learns to extract and separate the unbiased gender features and the semantic features from a gender-related utterance. The semantic features include all information of the utterance except unbiased gender features such as the content features and biased gender features. For the second challenge, we propose an adversarial learning framework to train bias-free generative dialogue models. Two discriminators are trained to distinguish the gender of a response based on its unbiased gender features and the semantic features, respectively. The dialogue model is trained with an objective to produce responses that can be distinguished correctly by the former and cannot be distinguished by the latter. In this way, unbiased gender features will be kept in the responses while biased gender features will be removed. We empirically validate the effectiveness of our proposed framework {\bf Debiased-Chat} by conducting experiments on two real-world dialogue datasets. Results show that our method can significantly mitigate the gender biases in generative dialogue models while maintaining the performance of the dialogue model to produce engaging and diverse responses with distinctive unbiased gender features.

% The rest of the paper is organized as follows. 
% First, we detail our proposed disentanglement model as well as the adversarial learning framework for bias-free dialogue generation in Section \ref{sec:method}. Next, we carries out our experimental setups and results with discussions in Section \ref{sec:exp}. Then, Section \ref{sec:relatedworks} reviews related works. Finally, Section \ref{sec:con} concludes the work with possible future research directions.


%We summarize our main contributions as follows:
%\begin{itemize}
 %   \item We identify the unbiased gender features and biased gender features of an utterance and propose a learning-based disentanglement approach to separate them for bias-free dialogue generation;
  %  \item We propose an adversarial learning based framework for bias-free dialogue generation, which keeps the distinctive unbiased gender features in responses and removes the biased gender features;
   % \item Extensive experiments are conducted on two real-world conversation corpora and demonstrate the effectiveness of our approach. We also validate the importance of the components in the proposed framework for high-quality bias-free dialogue generation.
%\end{itemize}

% Skeleton:

% 1. Fairness problems exist in many machine learning applications. Previous papers demonstrate that biases also exist in dialogue generation tasks. It's urgent for us to deal with it.

% 2. Some trivial methods can be used to solve the problem. The challenges of debiasing dialogue models. We don't want the responses for males and females to be the same. We only want the generated responses to be free from biased gender content while keeping the distinct unbiased gender characteristics in the responses. In this way, we can ensure that the dialogue model is still engaging and be able to produce diverse responses.

% 3. We focus on debiasing two classical types of dialogue models: a neural generative dialogue model and retrieval dialogue model. We propose a framework that trains dialogue models with adversarial training to mitigate gender bias. Besides, the optimization involving discrete text sampling is very difficult. We propose effective optimization techniques to train our framework. Experiment results show that our method successfully removes the bias while keeping the performance of the dialogue models to produce engaging responses.
